S-NeRF: Neural Radiance Fields for Street Views

Neural Radiance Fields (NeRFs) aim to synthesize novel views of objects and scenes, given the object-centric camera views with large overlaps. However, we conjugate that this paradigm does not fit the nature of the street views that are collected by many self-driving cars from the large-scale unbounded scenes. Also, the onboard cameras perceive scenes without much overlapping. Thus, existing NeRFs often produce blurs, 'floaters' and other artifacts on street-view synthesis. In this paper, we propose a new street-view NeRF (S-NeRF) that considers novel view synthesis of both the large-scale background scenes and the foreground moving vehicles jointly. Specifically, we improve the scene parameterization function and the camera poses for learning better neural representations from street views. We also use the the noisy and sparse LiDAR points to boost the training and learn a robust geometry and reprojection based confidence to address the depth outliers. Moreover, we extend our S-NeRF for reconstructing moving vehicles that is impracticable for conventional NeRFs. Thorough experiments on the large-scale driving datasets (e.g., nuScenes and Waymo) demonstrate that our method beats the state-of-the-art rivals by reducing 7% to 40% of the mean-squared error in the street-view synthesis and a 45% PSNR gain for the moving vehicles rendering.

==> figs_tex/ablation_background.tex <==
\begin{figure}[H] \label{fig:ablation}
\centering
\subfigure[w/o depth]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{figure/background/ablation_rgb.png}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[w/o depth confidence]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{figure/background/ablation_wof.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[w/o smooth loss]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{figure/background/ablation_nosmooth.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[Full Settings]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=1in]{figure/background/ablation_full.png}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{Ablation novel view synthesis}
\end{figure}


==> figs_tex/moving_cars.tex <==
\begin{figure}[H] \label{fig:moving_cars}
\centering
\subfigcapskip=5pt
\subfigbottomskip=2pt
\subfigure[GeoSim~\cite{geosim} \newline PSNR: 13.95]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figure/foreground/moving/geosim.pdf}
\end{minipage}%
}%
\subfigure[Ours \newline PSNR: 19.60]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figure/foreground/moving/ours.pdf}
\end{minipage}
}%
\subfigure[GT RGB]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figure/foreground/moving/gt.pdf}
%\caption{fig2}
\end{minipage}
}
\vspace{1mm}
\caption{Novel view synthesis comparison on moving car: (a) GeoSim can not synthesize a complete novel view on dynamic objects when the viewing angle changes drastically. (b) Our method produces a photorealistic novel view for moving vehicles. }
\vspace{2mm}
\end{figure}




==> file/tables/sup_efficiency.tex <==
\setlength{\tabcolsep}{10pt}
\renewcommand\arraystretch{1.3}
\begin{table}[t]
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{4pt}
%\vspace{-2mm}
\centering
\resizebox{0.7\textwidth}{!}{%

\begin{tabular}{lccc}
\toprule
Methods & PSNR & Time (hours) &  \# Params \\

\hline

Mip-NeRF ~\cite{mipnerf}& 18.22  &  & 9.0 \\

Mip-NeRF 360 ~\cite{mipnerf} & 24.37&  & 9.9  \\

Urban-NeRF ~\cite{urban-nerf}& 21.49 &   & 8.75 \\

\hline

Ours (no smooth) & 26.21 &  & 8.75 \\
Ours & 26.21 &  & 8.75 \\

\bottomrule
\end{tabular}
} 
\vspace{2mm}
\caption{Our method run 21h for 100K iters when applying smooth loss, and 17h without appling smooth loss, considering that the calculation of smooth loss needs extra patch samples} 
\vspace{-0.2em}
\label{tab:efficiency_background}

\end{table}

\iffalse
\setlength{\tabcolsep}{10pt}
\renewcommand\arraystretch{1.3}
\begin{table}[t]
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{4pt}
%\vspace{-2mm}
\centering
\resizebox{0.5\textwidth}{!}{%

\begin{tabular}{lccc}
\toprule
Methods & PSNR & Time (hours) &  \# Params \\

\hline

NeRF ~\cite{nerf} &  &  &  \\
\hline

Ours &  &  & \\

\bottomrule
\end{tabular}
} 
\vspace{2mm}
\caption{ Our method run faster than xxx?} 
\vspace{-0.2em}
\label{tab:efficiency_vehicles}

\end{table}
\fi
